Theory of Quantum Pulse Position Modulation and Related Numerical Problems

The paper deals with quantum pulse position modulation (PPM), both in the absence (pure states) and in the presence (mixed states) of thermal noise, using the Glauber representation of coherent laser radiation. The objective is to find optimal (or suboptimal) measurement operators and to evaluate the corresponding error probability. For PPM, the correct formulation of quantum states is given by the tensorial product of m identical Hilbert spaces, where m is the PPM order. The presence of mixed states, due to thermal noise, generates an optimization problem involving matrices of huge dimensions, which already for 4-PPM, are of the order of ten thousand. To overcome this computational complexity, the currently available methods of quantum detection, which are based on explicit results, convex linear programming and square root measurement, are compared to find the computationally less expensive one. In this paper a fundamental role is played by the geometrically uniform symmetry of the quantum PPM format. The evaluation of error probability confirms the vast superiority of the quantum detection over its classical counterpart.

==> KN/KN17.tex <==
% File: ./KN/KN17.tex creato da CA.m il {2009, 1, 27, 7, 39, 57.374251}
\l=103  \r=89  \unit=0.75mm
 % riga 1 di TeX

\xF=5 \where=2\xF=-58 \lD=110 \xD=4
% \grigliatrue

 % termine di TeX
 \Figura
 DIDASCALIA:Error probability in 3--PPM versus   the average number of photons
  per symbol $N_s$
 for  the  value  $\C(N)=0.1$ of the thermal noise parameter.  Solid line refers to SRM computation
 and dotted lines to convex linear programming (CLP) computation.
 INIZIO \put(0.80,61.24){\BP(102.60,84.36)
\put(-4.647,-73.326){\psfig{figure=./KN/KN17b.ps
,height=79.72mm,width= 121.2mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-58.743) AM=0.000  A=102.600  BM=60.260  B=84.364
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,23.10)(2,r,{{}}\relax)
% riga 1 di C1
\put(1,20.5){\circle*{0.6}}\put(2,19.4){\circle*{0.6}}
\put(3,18.5){\circle*{0.6}}\put(4,17.8){\circle*{0.6}}
\put(5,17.){\circle*{0.6}}\put(6,16.5){\circle*{0.6}}
\put(7,15.9){\circle*{0.6}}\put(8,15.2){\circle*{0.6}}
\put(9,14.5){\circle*{0.6}}\put(10,13.8){\circle*{0.6}}
\multiput(11,13.2)(1.,-0.51){20}{\circle*{0.6}}
\w(46.,2)[3,\C(N)=0.1\!\!\!]
%\WWW[10](66.5,-6)[2,d,\C(N)=0.2] \vet(66.5,4)(62.0,-7)
%\WWW[4](66.5,-22)[2,1,\C(N)=0.05]
%\circlepath1.5(75,-44)(92,-25)[0.5]
% termine aggiunte di C1
 \carattere=2 distanza=61.3
\sx 0.0 0,\sx 10.3 0.5,\sx 20.5 1,\sx 30.8 1.5,\sx 41.0 2,\sx 51.3 2.5,
 \sx 61.6 3,\sx 71.8 3.5,\sx 82.1 4,\sx 92.3 4.5,\sx 102.6 5,
\tacchex:p=-60.26 h=84.36 s=0.06 o=0.00 d=10.26 n=11
\tacchex:p=-60.26 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\tacchex:p=22.82 h=1.28 s=0.04 o=0.00 d=2.05 n=50
\carattere=2 distanza=1.0
\sy -60.3 10^{-7},\sy -48.2 10^{-6},\sy -36.2 10^{-5},\sy -24.1 10^{-4},\sy -12.1 10^{-3},\sy 0.0 10^{-2},
 \sy 12.1 10^{-1},\sy 24.1 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-60.26 d=12.05 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.63 d=12.05 n=7
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.63 d=12.05 n=7
\tacchey:p=0.00 h=1.28 s=0.04 o=-53.00 d=12.05 n=7
\tacchey:p=101.32 h=1.28 s=0.04 o=-53.00 d=12.05 n=7
\tacchey:p=0.00 h=1.28 s=0.04 o=-50.88 d=12.05 n=7
\tacchey:p=101.32 h=1.28 s=0.04 o=-50.88 d=12.05 n=7
\tacchey:p=0.00 h=1.28 s=0.04 o=-49.38 d=12.05 n=7
\tacchey:p=101.32 h=1.28 s=0.04 o=-49.38 d=12.05 n=7
{\linethickness{0.300\unitlength} \linR(0.00,-60.26,102.60)\linU(0.00,-60.26,84.36)
\linD(102.60,24.10,84.36)\linL(102.60,24.10,102.60)}
\W(97.47,-64.26)(2,c,{{N_s}}\relax)\W(-4.00,18.08)(2,r,{{P_e}}\relax)
 fine
 \EP}
 FINE


==> KN/KN19.tex <==
% File: ./KN/KN19.tex creato da CA.m il {2009, 1, 28, 7, 35, 2.615808}
\l=103  \r=90  \unit=0.75mm
 % riga 1 di TeX

\where=2 \xF=-58 \lD=110 \xD=4
% \grigliatrue

 % termine di TeX
 \Figura
 DIDASCALIA:Error probability in 3--PPM
  versus  the average number of photons per symbol
$N_s$ for some
 values of the thermal noise parameter $\C(N)$. Solid lines refer to quantum detection
 and dashed lines to classical photon counter detection.
 INIZIO \put(0.80,65.41){\BP(102.60,85.30)
\put(-4.647,-81.539){\psfig{figure=./KN/KN19b.ps
,height=83.13mm,width= 121.2mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C1
\rotw(68,-28.7)(-30)[2,\C(N)=0]
\rotw(69,-19.5)(-28)[2,\C(N)=0.05]
\rotw(69,-13.6)(-19)[2,\C(N)=0.1]\rotw(69,-7.3)(-18)[2,\C(N)=0.2]
%%%%%%%%%
\rotw(97,-17.2)(-20)[2,\C(N)=0]
\rotw(97,-13)(-25)[2,0.05]
\rotw(97,-7.3)(-22)[2,0.1]\rotw(97,-3)(-14)[2,\C(N)=0.2]
% termine aggiunte di C1
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{N_s}}\relax)\W(-4.00,15.99)(2,r,{{P_e}}\relax)
 fine
%
 %---------------- Curva N. 2 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 3 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3
\carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 4 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C4
% termine aggiunte di C4
\carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 5 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C5
% termine aggiunte di C4
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
 \EP}
 FINE


==> KN/KN25.tex <==
% File: ./KN/KN25.tex creato da CA.m il {2009, 1, 29, 18, 18, 28.877429}
\l=103  \r=90  \unit=0.75mm
 % riga 1 di TeX
 \where=2\xF=-58 \lD=110 \xD=4
% \grigliatrue

 % termine di TeX
 \Figura
 DIDASCALIA:Error probability in 4--PPM versus  the average number of photons per symbol
$N_s$ for some  values of  the thermal noise parameter $\C(N)$.
  Solid lines refer to quantum detection
 and dashed lines to classical photon counter detection.
 INIZIO \put(0.80,65.41){\BP(102.60,85.30)
\put(-4.647,-81.539){\psfig{figure=./KN/KN25b.ps
,height=83.132mm,width= 121.2mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
\rotw(68,-31.7)(-30)[2,\C(N)=0]
\rotw(69,-19.5)(-28)[2,\C(N)=0.05]
\rotw(69,-13.6)(-19)[2,\C(N)=0.1]\rotw(69,-7.3)(-18)[2,\C(N)=0.2]
% termine aggiunte di C1
% termine aggiunte di C1
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{N_s}}\relax)\W(-4.00,15.99)(2,r,{{P_e}}\relax)
 fine
%
 %---------------- Curva N. 2 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 3 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.33)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3
\carattere=2 distanza=65.0
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.98 h=85.30 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.98 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.04 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.0 10^{-8},\sy -53.3 10^{-7},\sy -42.7 10^{-6},\sy -32.0 10^{-5},\sy -21.3 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.3 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.98 d=10.66 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.77 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.56 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.68 d=10.66 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.35 d=10.66 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.98,102.60)\linU(0.00,-63.98,85.30)
\linD(102.60,21.33,85.30)\linL(102.60,21.33,102.60)}
\W(96.19,-67.98)(2,c,{{}}\relax)\W(-4.00,15.99)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 4 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
 fine
%
 %---------------- Curva N. 5 -------------
\Assi0(-0.800,-62.906) AM=0.000  A=102.600  BM=63.978  B=85.305
inizio
 fine
 \EP}
 FINE


==> KN/KN36.tex <==
% File: ./KN/KN36.tex creato da CA.m il {2009, 1, 27, 7, 54, 19.750921}
\l=103  \r=91  \unit=0.75mm
% riga 1 di TeX

\xF=-58 \where=2 \lD=110 \xD=4

%\grigliatrue
% termine di TeX

\Figura
DIDASCALIA: Error probability in 2--PPM versus  the average number of photons per symbol
$N_s$ for some  values of  the thermal noise parameter $\C(N)$. Comparison of SRM results with Helstrom's
      optimum results.
INIZIO \put(0.80,66.22){\BP(102.60,86.37)
\put(-4.647,-82.583){\psfig{figure=./KN/KN36b.ps1
,height=84.17mm,width= 121.2mm } }
\put(-4.647,-82.583){\psfig{figure=./KN/KN36b.ps2
,height=84.17mm,width= 121.2mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-63.716) AM=0.000  A=102.600  BM=64.778  B=86.370
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.59)(2,r,{{}}\relax)
\rotw(85,-33)(-24)[2,\C(N)=0.05]
\rotw(85,-44)(-34)[2,\C(N)=0]
\rotw(85,-12)(-18)[2,\C(N)=0.2]
\rotw(85,-20)(-25)[2,\C(N)=0.1]
\WWW[10](55.0,-5.5)[13,3,Helstrom]\WWW[10](45.0,-0.5)[13,3,SRM]
% riga 1 di C1
% termine aggiunte di C1
 \carattere=2 distanza=65.8
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.78 h=86.37 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.78 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.31 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.8 10^{-8},\sy -54.0 10^{-7},\sy -43.2 10^{-6},\sy -32.4 10^{-5},\sy -21.6 10^{-4},\sy -10.8 10^{-3},
 \sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.6 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.78 d=10.80 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.78,102.60)\linU(0.00,-64.78,86.37)
\linD(102.60,21.59,86.37)\linL(102.60,21.59,102.60)}
\W(96.19,-68.78)(2,c,{{N_s}}\relax)\W(-4.00,16.19)(2,r,{{P_e}}\relax)
 fine
%
 %---------------- Curva N. 2 -------------
\Assi0(-0.800,-63.716) AM=0.000  A=102.600  BM=64.778  B=86.370
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.59)(2,r,{{}}\relax)
% riga 1 di C2
% termine aggiunte di C2
 \carattere=2 distanza=65.8
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.78 h=86.37 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.78 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.31 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.8 10^{-8},\sy -54.0 10^{-7},\sy -43.2 10^{-6},\sy -32.4 10^{-5},\sy -21.6 10^{-4},\sy -10.8 10^{-3},
 \sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.6 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.78 d=10.80 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.78,102.60)\linU(0.00,-64.78,86.37)
\linD(102.60,21.59,86.37)\linL(102.60,21.59,102.60)}
\W(96.19,-68.78)(2,c,{{}}\relax)\W(-4.00,16.19)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 3 -------------
\Assi0(-0.800,-63.716) AM=0.000  A=102.600  BM=64.778  B=86.370
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.59)(2,r,{{}}\relax)
% riga 1 di C3
% termine aggiunte di C3
 \carattere=2 distanza=65.8
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.78 h=86.37 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.78 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.31 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.8 10^{-8},\sy -54.0 10^{-7},\sy -43.2 10^{-6},\sy -32.4 10^{-5},\sy -21.6 10^{-4},\sy -10.8 10^{-3},
 \sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.6 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.78 d=10.80 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.78,102.60)\linU(0.00,-64.78,86.37)
\linD(102.60,21.59,86.37)\linL(102.60,21.59,102.60)}
\W(96.19,-68.78)(2,c,{{}}\relax)\W(-4.00,16.19)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 4 -------------
\Assi0(-0.800,-63.716) AM=0.000  A=102.600  BM=64.778  B=86.370
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.59)(2,r,{{}}\relax)
% riga 1 di C4
% termine aggiunte di C4
 \carattere=2 distanza=65.8
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.78 h=86.37 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.78 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.31 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.8 10^{-8},\sy -54.0 10^{-7},\sy -43.2 10^{-6},\sy -32.4 10^{-5},\sy -21.6 10^{-4},\sy -10.8 10^{-3},
 \sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.6 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.78 d=10.80 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.78,102.60)\linU(0.00,-64.78,86.37)
\linD(102.60,21.59,86.37)\linL(102.60,21.59,102.60)}
\W(96.19,-68.78)(2,c,{{}}\relax)\W(-4.00,16.19)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 5 -------------
\Assi0(-0.800,-63.716) AM=0.000  A=102.600  BM=64.778  B=86.370
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.59)(2,r,{{}}\relax)
% riga 1 di C5
% termine aggiunte di C5
 \carattere=2 distanza=65.8
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.78 h=86.37 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.78 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.31 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.8 10^{-8},\sy -54.0 10^{-7},\sy -43.2 10^{-6},\sy -32.4 10^{-5},\sy -21.6 10^{-4},\sy -10.8 10^{-3},
 \sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.6 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.78 d=10.80 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.78,102.60)\linU(0.00,-64.78,86.37)
\linD(102.60,21.59,86.37)\linL(102.60,21.59,102.60)}
\W(96.19,-68.78)(2,c,{{}}\relax)\W(-4.00,16.19)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 6 -------------
\Assi0(-0.800,-63.716) AM=0.000  A=102.600  BM=64.778  B=86.370
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.59)(2,r,{{}}\relax)
% riga 1 di C6
% termine aggiunte di C6
 \carattere=2 distanza=65.8
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.78 h=86.37 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.78 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.31 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.8 10^{-8},\sy -54.0 10^{-7},\sy -43.2 10^{-6},\sy -32.4 10^{-5},\sy -21.6 10^{-4},\sy -10.8 10^{-3},
 \sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.6 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.78 d=10.80 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.78,102.60)\linU(0.00,-64.78,86.37)
\linD(102.60,21.59,86.37)\linL(102.60,21.59,102.60)}
\W(96.19,-68.78)(2,c,{{}}\relax)\W(-4.00,16.19)(2,r,{{}}\relax)
 fine
%
 %---------------- Curva N. 7 -------------
\Assi0(-0.800,-63.716) AM=0.000  A=102.600  BM=64.778  B=86.370
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.59)(2,r,{{}}\relax)
% riga 1 di C7
% termine aggiunte di C7
 \carattere=2 distanza=65.8
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.78 h=86.37 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.78 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.31 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.8 10^{-8},\sy -54.0 10^{-7},\sy -43.2 10^{-6},\sy -32.4 10^{-5},\sy -21.6 10^{-4},\sy -10.8 10^{-3},
 \sy 0.0 10^{-2},\sy 10.8 10^{-1},\sy 21.6 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.78 d=10.80 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-61.53 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-58.28 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-56.38 d=10.80 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.03 d=10.80 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.78,102.60)\linU(0.00,-64.78,86.37)
\linD(102.60,21.59,86.37)\linL(102.60,21.59,102.60)}
\W(96.19,-68.78)(2,c,{{}}\relax)\W(-4.00,16.19)(2,r,{{}}\relax)
 fine
 \EP}
 FINE


==> KN/KN50.tex <==









% File: ./KN/KN50.tex creato da CA.m il {2009, 1, 27, 7, 58, 56.053062}
\l=103  \r=90  \unit=0.75mm
 % riga 1 di TeX

% \grigliatrue
 \where=2 \xF=-58 \lD=110 \xD=4
 % termine di TeX
 \Figura
 DIDASCALIA:Error probability of classic and quantum
            2--PPM in the absence of thermal noise.
         $N_s$ is the average number of photons per symbol.                                                            INIZIO \put(0.80,66.22){\BP(102.60,85.52)
\put(-4.647,-91.493){\psfig{figure=./KN/KN50b.ps
,height=91.5mm,width= 121.2mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-63.721) AM=0.000  A=102.600  BM=64.139  B=85.519
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.38)(2,r,{{}}\relax)
% riga 1 di C1
\w(71,-4)[13,classic]
\w(66,-27)[13,quantum]
% termine aggiunte di C1
 \carattere=2 distanza=65.1
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-64.14 h=85.52 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-64.14 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=20.10 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -64.1 10^{-8},\sy -53.4 10^{-7},\sy -42.8 10^{-6},\sy -32.1 10^{-5},\sy -21.4 10^{-4},\sy -10.7 10^{-3},
 \sy 0.0 10^{-2},\sy 10.7 10^{-1},\sy 21.4 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-64.14 d=10.69 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.92 d=10.69 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.92 d=10.69 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.70 d=10.69 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.70 d=10.69 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.82 d=10.69 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.82 d=10.69 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.49 d=10.69 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.49 d=10.69 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-64.14,102.60)\linU(0.00,-64.14,85.52)
\linD(102.60,21.38,85.52)\linL(102.60,21.38,102.60)}
\W(96.19,-68.14)(2,c,{{N_s}}\relax)\W(-4.00,16.03)(2,r,{{P_e}}\relax)
 fine
 \EP}
 FINE


==> KN/KN52.tex <==
% File: ./KN/KN52.tex creato da CA.m il {2009, 1, 27, 8, 2, 18.024113}
\l=103  \r=89  \unit=0.75mm
 % riga 1 di TeX

% \grigliatrue
 \where=2 \xF=-58 \lD=110 \xD=4
 % termine di TeX
 \Figura
 DIDASCALIA:Error probability  versus  the average number of photons per symbol
$N_s$ of classic and quantum
            3--PPM in the absence of thermal noise.                                                            INIZIO \put(0.80,63.89){\BP(102.60,84.93)
\put(-4.647,-84.106){\psfig{figure=./KN/KN52b.ps
,height=88.71mm,width= 121.2mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-61.387) AM=0.000  A=102.600  BM=63.700  B=84.933
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.23)(2,r,{{}}\relax)
% riga 1 di C1
\w(83,-5)[13,classic]
\w(71,-27)[13,quantum]
% termine aggiunte di C1
 \carattere=2 distanza=64.7
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.70 h=84.93 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.70 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=19.95 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -63.7 10^{-8},\sy -53.1 10^{-7},\sy -42.5 10^{-6},\sy -31.8 10^{-5},\sy -21.2 10^{-4},\sy -10.6 10^{-3},
 \sy 0.0 10^{-2},\sy 10.6 10^{-1},\sy 21.2 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.70 d=10.62 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.50 d=10.62 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.50 d=10.62 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.31 d=10.62 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.31 d=10.62 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.44 d=10.62 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.44 d=10.62 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-54.11 d=10.62 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-54.11 d=10.62 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.70,102.60)\linU(0.00,-63.70,84.93)
\linD(102.60,21.23,84.93)\linL(102.60,21.23,102.60)}
\W(96.19,-67.70)(2,c,{{N_s}}\relax)\W(-4.00,15.92)(2,r,{{P_e}}\relax)
 fine
 \EP}
 FINE


==> KN/KN54.tex <==
% File: ./KN/KN54.tex creato da CA.m il {2009, 1, 27, 8, 3, 25.815752}
\l=103  \r=89  \unit=0.75mm
 % riga 1 di TeX

%\grigliatrue

 \where=2 \xF=-58 \lD=110 \xD=4
 % termine di TeX
 \Figura
 DIDASCALIA:Error probability  versus  the average number of photons per symbol
$N_s$ of classic and quantum
            4--PPM in the absence of thermal noise.                                                            INIZIO \put(0.80,62.73){\BP(102.60,84.67)
\put(-4.647,-80.040){\psfig{figure=./KN/KN54b.ps
,height=86.88mm,width= 121.2mm } }
%
 %---------------- Curva N. 1 -------------
\Assi0(-0.800,-60.234) AM=0.000  A=102.600  BM=63.505  B=84.674
inizio
\W(101.60,-1.50)(2,t,{{}}\relax)
\W(-1.50,20.17)(2,r,{{}}\relax)
% riga 1 di C1
\w(83,-5)[13,classic]
\w(68,-23)[13,quantum]
% termine aggiunte di C1
 \carattere=2 distanza=64.5
\sx 0.0 0,\sx 12.8 1,\sx 25.6 2,\sx 38.5 3,\sx 51.3 4,\sx 64.1 5,
 \sx 77.0 6,\sx 89.8 7,\sx 102.6 8,
\tacchex:p=-63.51 h=84.67 s=0.06 o=0.00 d=12.82 n=9
\tacchex:p=-63.51 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\tacchex:p=19.89 h=1.28 s=0.04 o=0.00 d=2.56 n=40
\carattere=2 distanza=1.0
\sy -63.5 10^{-8},\sy -52.9 10^{-7},\sy -42.3 10^{-6},\sy -31.8 10^{-5},\sy -21.2 10^{-4},\sy -10.6 10^{-3},
 \sy 0.0 10^{-2},\sy 10.6 10^{-1},\sy 21.2 10^{0},
\tacchey:p=0.00 h=102.60 s=0.06 o=-63.51 d=10.58 n=9
\tacchey:p=0.00 h=1.28 s=0.04 o=-60.32 d=10.58 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-60.32 d=10.58 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-57.13 d=10.58 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-57.13 d=10.58 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-55.27 d=10.58 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-55.27 d=10.58 n=8
\tacchey:p=0.00 h=1.28 s=0.04 o=-53.95 d=10.58 n=8
\tacchey:p=101.32 h=1.28 s=0.04 o=-53.95 d=10.58 n=8
{\linethickness{0.300\unitlength} \linR(0.00,-63.51,102.60)\linU(0.00,-63.51,84.67)
\linD(102.60,21.17,84.67)\linL(102.60,21.17,102.60)}
\W(96.19,-67.51)(2,c,{{N_s}}\relax)\W(-4.00,15.88)(2,r,{{P_e}}\relax)
 fine
 \EP}
 FINE


==> bkq.tex <==
\bozzefalse
\begin{small}

\Bibliografario(BB){References}


%[10]
\noindent\J(Glauber) R.J. Glauber, ``Coherent and incoherent states of the
radiation field'', {\it Phys. Rev.}, vol. 131, pp. 2766--2788, Sep.
1963.


\J(Rakosi) A. Lee, ``Note on the spectra of finite permutation
matrices'', {\it Publications Mathematical (Debrecen)},
vol. 14, pp. 75--78, 1967.

%[14]
\J(Helstrom) C.W. Helstrom, J.W.S. Liu, and J.P. Gordon, ``Quantum mechanical
communication theory'', {\it Proceedings of the IEEE}, vol. 58, no.
10, pp. 1578--1598, Oct. 1970.

\J(Kennedy) R.S. Kennedy, ``A near--optimum 
receiver for the binary coherent state quantum channel'',
 {\it MIT Research Laboratory of Electronics, Quartely 
 Progress Report 108}, Cambridge, pp. 219--225, \me1, 1973.




\J(Dolinar) S.J. Dolinar, Jr., ``An optimum receiver
 for the binary coherent state
quantum
channel'',  {\it MIT Research Laboratory of Electronics
 Quarterly Progress
Report
111}, Massachussetts Institute of Technology, Cambridge, 
Massachussetts,
pp. 115--120, \me10, 1973.


%[2]
\J(Holevo) A.S. Holevo, ``Statistical decision theory for quantum systems'',
{\it J. Multivar. Anal.}, vol. 3, pp. 337--394, Dec. 1973.

%[3]
\J(Yuen) H.P. Yuen, R.S. Kennedy, and M. Lax, ``Optimum testing of
multiple hypotheses in quantum detection theory'', {\it IEEE
Trans. Inform. Theory}, vol. IT--21, pp. 125--134, Mar. 1975.

%[1]
\J(Helstrom2) C.W. Helstrom. {\it Quantum Detection and Estimation Theory}.
New York: Academic Press, 1976.


\J(Henderson) H.V. Henderson and S.R. Searle,
 ``The vec permutation matrix, the vec operator and Kronecker products:
 a review'', {\it Linear and Multilinear Algebra}, vol. 9, pp. 271--288,
 Jan. 1981.
 
\J(Dolinar2) S.J. Dolinar,
  Jr, ''A near--optimum receiver structure for the detection
   of $M$--ary optical PPM signals'', {\it JPL TDA Prog. Rep.},
    vol. 42--72, pp. 30--42, Feb. 1983.

\J(Horn2)    R. Horn and C. Jonhson, {\it Topics in Matrix Analysis}.
      Cambridge   Cambridge University Press, 1989, Chapter 4.
%[8]
\J(Hausladen) P. Hausladen, R. Josza, B. Schumacher, M. Westmoreland, and
W.K. Wootters, ``Classical information capacity of a quantum
channel'', {\it Phys. Rev. A}, vol. 54, pp. 1869--1876, Sept. 1996.

\J(Ban1997) M. Ban, K. Kurokawa, R. Momose, and O. Hirota, ``Optimum
measurements for discrimination among symmetric quantum state and
parameter estimation'', {\it Int. J. Theor. Phys.}, vol. 36, pp.
1269--1288, 1997.
 
%[11]
\J(Sasaki) M. Sasaki, R. Momose, and O. Hirota, ``Quantum
detection for an on--off keyed mixed--state signal with a small amount of
thermal noise'', {\it Phys. Rev. A}, vol. 55, pp. 3223--3226, April 1997.

\J(Horn) R. A. Horn and C.R. Johnson. {\it Matrix Analysis}. Cambridge: 
Cambridge University Press, 1998.


\J(Kato1999) K. Kato, M. Osaki, M. Sasaki, and O. Hirota, ``Quantum
detection and mutual information for QAM and PSK signals'', {\it
IEEE Trans. on Commun.}, vol. COM--47, pp. 248--254, Feb. 1999.

%[6]


\J(Chefles) A. Chefles, ``Quantum State Discrimination'',
 {\it Contemporary Physics}, vol. 41, pp. 401--424, 2000.
 
%[7]
\J(Forney1) Y.C. Eldar and G.D. Forney, Jr., ``On quantum detection and
the square--root measurement'', {\it IEEE Trans. Inform. Theory},
vol IT--47, pp. 858--872, Mar. 2001.


\J(Vilrotter) V.A. Vilnrotter and C.--W. Lau, ``Quantum detection of binary
and ternary signals in the presence of thermal noise fields'', {\it The
Interplanetary Network Progress Report} No. 42--152, Feb. 2003.



%[5]
\J(Eldar2003)  Y.C. Eldar, A. Megretski, and G.C. Verghese, ``Designing
optimal quantum detectors via semidefinite programming'', {\it
IEEE Trans. Inform. Theory}, vol IT--49, pp. 1007--1012, Apr.
2003.




%[9]
\J(Eldar3)  Y.C. Eldar, A. Megretski, and G.C. Verghese, ``Optimal
detection of symmetric mixed quantum states'', {\it IEEE Trans. Inform. Theory}, 
vol IT--50, pp. 1198--1207, June 2004.

\J(JPLbook) S.J. Dolinar, J. Hamkins, B.E. Moision, and  V.A. Vilnrotter,
 ``Optical modulation and coding'' in H. Hemmati (Ed),
 {\it Deep Space Optical Communications}. New York: Wiley, 2006.


 

 \J(Nature) R.L. Cook, P.J. Martin, and J.M. Geremia,
 ``Optical coherent state discrimination using a 
 closed--loop quantum measurement'', {\it Nature}, vol.446,
 pp. 774--777, April 2007.
%[12]




\J(CarPier) G. Cariolaro and G. Pierobon, ``Performance of quantum
data transmission systems in the presence of thermal noise'',
it will be published on {\it
IEEE Trans. on Commun.}, Feb. 2010. Available: 
          http//www.arXiv.org/abs/quant--ph/0904.1073.
\end{small}


==> kq1.tex <==

\def\bk(#1,#2){\langle#1|#2\rangle}
\def\bok(#1,#2,#3){\langle#1|#2|#3\rangle}
\def\kb(#1,#2){|#1\rangle\langle#2|}
\def\lb{\lambda}
\def\ket(#1){|#1\rangle}
\def\k(#1){\ket(#1)}
\def\mod{\ {\rm mod}\ }
\def\rank(#1){{\rm rank}\,(#1)}
\def\Tr{{\rm Tr}}

\thispagestyle{empty}


%\figfalse
%\tabfalse

\bozzefalse

%\newpage
\begin{abstract}
The paper deals with  quantum pulse position modulation (PPM),
both in the absence (pure states) and in the presence (mixed states)
of thermal noise, using the Glauber representation of coherent
laser radiation.  The objective is to find optimal
(or suboptimal)
measurement operators  and to evaluate the corresponding error probability.
For  PPM, the correct formulation of quantum states is given
by the tensorial product of $m$ identical Hilbert spaces, where $m$ is
the PPM order. The presence of mixed states, due to thermal noise,
generates an optimization problem involving matrices
 of huge dimensions, which already for 4--PPM, are of the order of ten
thousand. To overcome this computational complexity,
 the currently available methods of quantum detection, which are based on explicit results,
convex linear programming and square root measurement, are compared to find
the  computationally less expensive one. In this paper a fundamental role is played by the
geometrically uniform symmetry of the quantum PPM format.
The  evaluation of error probability confirms the vast superiority of the
quantum detection over its classical counterpart.
\end{abstract}
\begin{keywords} Quantum detection, linear programming, square root measurement
 (SRM), least square measurement (LSM), geometrically
uniform symmetry (GUS), thermal noise, pulse position modulation (PPM).
\end{keywords}



\section{Introduction}

Coherent optical communications  represent
the best way to convey an enormous amount of information over large distances,
 both through fibers
and in free space. Quantum
optical communications offer the possibility to improve
the performance of (classical) optical communications by basing the design
of the detection on the laws of Quantum Mechanics. Several authors
have shown, both theoretically \bibl(Helstrom)\bibl(Kato1999)\bibl(CarPier)
 and experimentally \bibl(Kennedy)\bibl(Dolinar)\bibl(Vilrotter)\bibl(Nature),
 that  improvements, of at least a decade, can be obtained
 in terms of error  probability.
 The uncertainty in quantum detection
 is intrinsically
linked to the laws of quantum mechanics. In the language of
classical optical systems, this uncertainty corresponds to the
so called {\it shot noise}. Another source of uncertainty is the
presence of {\it thermal noise}.

Necessary and sufficient conditions
for the optimal measurement set were found in pioneering
papers by Holevo \bibl(Holevo) and  Yuen {\it et al.} \bibl(Yuen).
Although the optimal measurement set is
completely characterized, explicit solutions for
the optimal measurement set are in general
not available. It is therefore necessary to resort to a
numerical evaluation based on convex semidefinite programming \bibl(Eldar2003).
However, under a certain symmetry constraint, called {\it geometrically
uniform symmetry} (GUS),
a simple measurement, introduced by Hausladen {\it et al.}
\bibl(Hausladen),  and known as {\it
square root measurement} (SRM), turns out to be optimum. This SRM has
the  remarkable advantage that, starting from the given states,
 it can be straightforwardly evaluated. Moreover, even when
it is not optimal, the SRM  often provides ``pretty good'' upper bounds on
the performance of optimal detectors.

The
problem of quantum detection in a noisy environment has received
scarce  attention in the literature, but
the extension of SRM to mixed states \bibl(Eldar3)
 has opened new perspectives.
  In a previous paper \bibl(CarPier),  we applied this extension to
 the analysis of quantum communication systems, in the presence of
 thermal noise, using the Glauber theory on coherent states \bibl(Glauber)
to represent the noisy quantum  channel.


In this paper,  the theory of \bibl(CarPier), which was applied to PSK (phase
shift keying) and
QAM (quadrature amplitude modulation) systems,  will be
extended to PPM (quantum pulse position
modulation)  systems. The novelty of this modulation format
is that it  must be formulated (see
\bibl(Yuen)\bibl(Vilrotter)) in a composite
Hilbert space $\C(H)$, given by the tensor product
 $\C(H)_0^{\otimes m}$ of $m$ identical
  Hilbert spaces $\C(H)_0$, where $m$ is the   PPM's alphabet size. Thus,
  the quantum states corresponding to the classical binary
  PPM symbols are given by  the tensor product
of $m$ Glauber coherent  states. For instance,
 in   4--PPM, the  composite states representing
the symbols $[0001],[0010],[0100],[1000]$,   are given by
$$
\eqalign{
|\gamma_0\rangle&=|0\rangle\!\otimes\!|0\rangle\!\otimes\!|0\rangle\!\otimes\!
        |\alpha\rangle
  \q|\gamma_1\rangle=|0\rangle\!\otimes\!|0\rangle\!\otimes\!|\alpha\rangle|
  \!\otimes\!0\rangle\cr
|\gamma_2\rangle&=|0\rangle\!\otimes\!|\alpha\rangle\!\otimes\!|0\rangle\!\otimes\!
          |0\rangle
\q|\gamma_3\rangle=|\alpha\rangle\!\otimes\!|0\rangle\!\otimes\!|0\rangle\!\otimes\!|
0\rangle\cr}
\e(W5)
$$
where the symbol 1 is represented by a Glauber state $|\alpha\rangle$,
with an average number of
photons given by $ N_s=|\alpha|^2$,
 and the symbol 0 by
the  Glauber ``ground state''  $|0\rangle$, which has zero photons.
In the presence of noise (mixed states) the $m$ composite states
must be replaced by $m$ composite density operators.
If  $n$ is the dimension of the basic Hilbert space $\C(H)_0$, the dimension
of  the composite space $\C(H)=\C(H)_0^{\otimes m}$ becomes $N=n^m$, which
gives rise to  a problem
of computational complexity. In the approximation of the Glauber
representation, in order to guarantee an adequate approximation, the choice of
dimension $n$ (theoretically infinite) depends
on the  average number of photons $N_s$, which
 in turn depends on the range of the error probability $P_e$ that
we wish to explore. To fix  ideas, we anticipate the following schedule
for  4--PPM
\bu  $P_e\simeq 10^{-2}\;\arr\,\, N_s\simeq3\;\;\;\arr\,\, n\simeq 10\vl N=n^m\simeq\,\,10^4$
\bu  $P_e\simeq 10^{-3}\;\arr\,\, N_s\simeq4.5\arr\,\, n\simeq 15\vl N=n^m\simeq\,5 \;10^4$
\bu  $P_e\simeq 10^{-4}\;\arr\,\, N_s\simeq6.5\arr\,\, n\simeq 20\vl N=n^m\simeq16\;10^4$


\ET Thus, we realize that, while the dimension $n$ of  basic space can be
confined to moderately small values, the dimension $N$ of  composite
space quickly becomes   huge  with consequently severe
numerical problems, mainly related to the
eigendecomposition (EID) of $N\times N$ matrices. Therefore, one of
the main targets of the paper will be a systematic comparison
of the currently available methods,  to find the lowest
computational complexity and, where possible,
to search for analytical results for which the numerical evaluation
does not represent a problem for any arbitrarily large dimension
(see the EID of the PPM symmetry operator in Section III).

The above schedule refers  to a moderate
amount of thermal noise ($\C(N)=0.05$ thermal noise photons). Note that
in the absence of noise, that is with pure states, the analysis
is straightforward and the error probability is known, in closed form,
from the pioneering works of Yuen, Kennedy and Lax \bibl(Yuen),
 although the authors do not mention applications to PPM.

This paper is organized as follows. In Section II we give a detailed overview
of the quantum detection problem.  In Section III we formulate the theory of PPM
and prove that the  quantum PPM format satisfies the
 GUS property, which  surprisingly enough, has not been
noticed elsewhere; the main task is to find an analytical expression for
the symmetry operator and its EID. In Section IV we formulate the
PPM quantum states according to the Glauber theory. Finally, in Section V,
after a comparative discussion of  computational complexity, we evaluate the PPM
performances, up to the order $m=4$. In Section VI we mention to
the problem of implementation.


\vspace{-2mm}

\Paragrafo(RV){Overview of Quantum Detection}

This overview is finalized to PPM. For a general overview, see \bibl(CarPier).



\vspace{-2mm}


\subsection{Formulation of the problem}

The quantum detection problem is stated as follows \bibl(Helstrom).
A transmitter conveys classical information to a receiver through
 a quantum--mechanical channel, by choosing a quantum state from a
  set $\{\rho_i| i=0,\dots,m-1\}$ of {\co density operators}
   on an $N$--dimensional Hilbert space $\C(H)$.
   The density operators
 $\rho_i$ are chosen  with  given {\co prior probabilities}
  $q_i$, but  in what follows, we assume equal probabilities, i.e.,  $q_i=1/m$.
The receiver detects the transmitted information with a set of
 {\co positive operator valued measurements} (POVM)
$\Pi_0,\ldots,\Pi_{m-1}$.
 Provided that the state density operator is $\rho_i$,
  the probability that  the detection system reveals the state $j$,
  is given by the transition probability
$
p(j|i)=\Tr(\rho_i\Pi_j)$, $ i,j=0,\ldots,m-1
$.
Then, the probability of correct detection becomes
$$
P_c={1\over m}\sum_{i=0}^{m-1}p(i|i)={1\over m}\sum_{i=0}^{m-1}\Tr(\rho_i\Pi_i)\;.\e(R2)
$$
The description through density operators represents
 the general case, and includes  the pure state case,
 in which
 $\rho_i$ reduces to the rank--one
operator
$
\rho_i=\kb(\gamma_i,\gamma_i)
$.


Quantum detection   is simplified and has specific properties if the state
 constellation
 exhibits the  Geometrically Uniform Symmetry (GUS), that  is
if  a unitary operator $S$ exists with the properties%
  \footnote{In this formulation equal prior probabilities are implied. In
  the general case, the {\it weighted} density operators $q_i\rho_i$
  should be considered \bibl(Eldar3). Note that if the GUS holds with
  equal probabilities, as in \e(,R13), it does not hold with arbitrary
  probabilities.}
$$
\rho_i=S^i\rho_0S^{-i}  \vq S^m=I_\C(H)
\e(R13)
$$
where $S$ is
the {\it symmetry operator},
and  $\rho_0$ is the {\it generating density operator}.
The simplifications with  GUS are:
 1) The quantum source is completely specified by $\rho_0$  and $S$.
 2) The POVM $\Pi_i$ can be chosen to have the same GUS as
     the density operators $\rho_i$ \bibl(Eldar3), namely,
     $
      \Pi_i=S^i\,\Pi_0\,S^{-i}
      $.
     The search can then be limited to the reference POVM $\Pi_0$.
 3) The transition probabilities $p(j|i)$ depend only on
      the difference $i-j$, mod $m$ (their matrix is circulant). In fact,
      $p(j|i)=\Tr\left[\Pi_0\,S^{i-j}\,\rho_0\,S^{-(i-j)}\right]$.
      Consequently
      $$
      P_c=\Tr(\rho_0\Pi_0)\,.
      \e(R27)
      $$

The positive semidefinite (PSD) Hermitian operators $\rho_0$ and $\Pi_0$ may, in some respect,
 be redundant and can then be
investigated through their {\it factors}. In an $N$--dimensional Hilbert space
the density operators $\rho_0$ are represented by $N\times N$ complex matrices
and can be factorized in the form
 $\rho_0=\gamma_0\gamma_0^*$, where $\gamma_0$ is a convenient $N\times r_0$
 matrix, with $r_0=\rank(\rho_0)$.
  This factorization
is not unique, but the ambiguity turns out to be irrelevant in  quantum
detection \bibl(Eldar3).
  In particular, if the states are pure, then $r_0=1$ and $\gamma_0$ reduces to
   the ket $\k(\gamma_0)$.
Since the rank of the optimal POVM  $\Pi_0$ is not greater
 than $r_0$ \bibl(Eldar3), we postulate a similar factorization
 $\Pi_0=\mu_0\mu_0^*$
 of the measurement operator. In the presence of GUS the factors
 of $\rho_i$ and $\Pi_i$ can be obtained from the reference factors
 as
    $
      \gamma_i=S^i\,\gamma_0  $ and $  \mu_i=S^i\,\mu_0$,
     where $\gamma_i$ and $\mu_i$ have the same dimension $N\times r_0$.




\subsection{Optimal solution (minimum error probability)}


In their pioneering papers, Holevo \bibl(Holevo) and Yuen {\co et al.} \bibl(Yuen)
 found
necessary and sufficient conditions (see also \bibl(Eldar3)) for an optimum
 POVM set (which minimized the error probability).
In a few special cases, the optimal POVM set is explicitly known, namely:
 1) for binary systems in the general case of mixed states,
 and 2) for $m$-ary systems with pure states
 having  GUS. Case 2) will be seen
 below in the context of SRM. Case 1) is due to Helstrom \bibl(Helstrom),
 who obtained the following explicit result:
 \smallskip
 \Proposition(Hel) Let $\rho_0$ and $\rho_1$ be the density operators of a binary
 quantum system. Define the decision
 operator $D=q_1\rho_1-q_0\rho_0$, where $q_0$ and $q_1$  are the
  prior probabilities,  and find the corresponding EID:
 $D=\sum_i \epsilon_i|\epsilon_i\rangle\langle \epsilon_i|$, where the eigenvalues
 $\epsilon_i$ are real and $|\epsilon_i\rangle$  are the corresponding
eigenvectors. Then, the optimal POVM are given by
 $\Pi_0=\sum_{ \epsilon_i\leq0}|\epsilon_i\rangle\langle \epsilon_i|$ and
  $\Pi_1=\sum_{ \epsilon_i>0}|\epsilon_i\rangle\langle \epsilon_i|$. The
  corresponding correct detection probability  is given  by
  $P_c=q_0+\sum_{ \epsilon_i>0}\epsilon_i$.
 \endprop


In the general case, explicit solutions for the optimal POVM
  are not available. However, the problem
 of  maximizing the correct detection probability $P_c$ can be solved numerically
 by {\it convex semidefinite programming} \bibl(Eldar2003).
 For instance, one can use the
 LMI (Linear Matrix Inequality) Toolbox of MatLab,
 which permits evaluating the optimal performance   with
any desired accuracy.
 Of course, if the dimensions are very large,
   as in the case of PPM with mixed states, the numerical evaluation may become very time
   and storage consuming.





\subsection{SRM solution (square root measurement)}

A more straightforward, although not optimal, approach to the
 problem is offered by the SRM.  The approach   for pure states  was proposed
   by Hausladen {\it et al.} \bibl(Hausladen)
   and thoroughly investigated by Eldar and Forney \bibl(Forney1).
 The generalization to mixed states is due to Eldar {\co et al.} \bibl(Eldar3).
 In the last paper it is shown that  SRM is equivalent
 to LSM (least square measurement).
The SRM formulation is stated in terms of   the {\co state matrix}
$
\Gamma=\qmatrix{\gamma_0,\gamma_1,\ldots,
\gamma_{m-1}\cr}
$
and of
the {\co measurement
matrix}
$
M=\qmatrix{\mu_0,\mu_1,\ldots,\mu_{m-1}\cr}
$, both of dimension $N\times m\,r_0$.  Now, the quantum
detection problem can be reformulated in terms of the matrix $\Gamma$
(given) and  the matrix $M$ (to be found).

\smallskip
 \Proposition(SRM) (see \bibl(Forney1)) In the SRM the measurement matrix $M$ is given by the two
 equivalent expressions
 $$
   M=T^{-1/2}\,\Gamma\vq  M=\Gamma\,G^{-1/2}
   \e(Z2)
$$
where $T^{-1/2}$ and $G^{-1/2}$ are the inverse square roots
(in the Moore--Penrose generalized sense) of $T$ and $G$, respectively.
\endprop
\smallskip

\ET The alternative approaches to evaluate $M$, either via $T^{-1/2}$ or via $G^{-1/2}$,
are  important
 for  efficient computation.
We develop these results in the case of GUS, which is of special interest
for PPM. The first of \e(Z2) gives  the reference POVM as
$
 \Pi_0=T^{-1/2}\,\rho_0\,T^{-1/2}
$.
Once  $ T^{-1/2} $ is evaluated, we can obtain the transition probabilities, and
  then the correct detection probability from \e(R27), which becomes
 $$
 P_c=\Tr\left[(\rho_0T^{-1/2})^2\right]\,.
 \e(Z6)
 $$

The Gram matrix approach is less direct. The matrix
$G$ is block circulant  and its decomposition
is related to the discrete Fourier transform (DFT). In \bibl(CarPier)
we found:

\smallskip
\Proposition(DFT) In the presence of GUS the $i,j$ block of the
Gram matrix, of size $r_0\times r_0$, can be written in the form
$$
G_{ij}=\gamma_i^*\gamma_j=\gamma_0^*S^{j-i}\gamma_0=
{1\over m}\sum_{k=0}^{m-1}W_m^{k(j-i)}E_k
\e(Z16)
$$
where $W_m=e^{i2\pi/m}$ and the matrices $E_k$, of order $H$, have the alternative expressions
$$
E_k=m\gamma_0^*\,Y_k\,\gamma_0=\sum_{i=0}^{m-1}G_{0i}W_m^{-ki}\,.
\e(Z18)
$$
Here,  $Y_k$ are the matrices appearing in the EID of $S$ (see \e(,S13)).
The correct detection probability is finally given by
$$
P_c=\frac1m\Tr\Bigl[\Bigl\{
          \sum_{k=0}^{m-1}E_k^{1/2}\Bigr\}^2\,\Bigr]\,.
\e(P25)
$$
\endprop




\smallskip

In conclusion, with the Gram matrix approach, the performance
evaluation requires  finding the square roots $E_k^{1/2}$, by the EID,
of the $r_0\times r_0$
matrices $E_k$ defined by \e(Z18).

\ev{SRM optimality with GUS} Under certain conditions,  SRM provides the optimal
solution for the general case of mixed states. A (sufficient) condition is that
the state constellation has  GUS and the reference factors satisfy
the relation \bibl(Eldar3)
$\mu_0^*\,\gamma_0= \alpha \;I_H$,
where $\alpha$ is an arbitrary constant. Unfortunately, for  PPM this condition
holds only for pure states.



\vskip-2mm


\Paragrafo(QPPM){Quantum Pulse Position Modulation (QPPM)}

\iffalse
QPPM  is an attractive modulation format, which has recently been considered
\bibl(JPLbook) for possible applications to deep space
communications. However, the model of QPPM we consider
below is a paradigm for a whole class of different
quantum communication schemes. For instance, it has been proved
\bibl(Helstrom) that the model is the quantum--mechanical
equivalent of a general communication system with (classically)
orthogonal waveforms.
\fi

QPPM is an attractive modulation format, which has recently been considered
\bibl(JPLbook) for possible applications to deep space communications.
Indeed, it
 appears well suited to existing laser modulation techniques, in that it
 can be regarded as a coded version of the OOK format. In particular the
  requirements for the transmitting laser are the same as for the OOK
   coherent modulation, with lower average power. On the other hand, the
    model of the QPPM we consider below is a paradigm for a whole class
     of quantum communication scheme (as wavelength modulation). Moreover,
     it has been proved [3] that the model is a quantum--mechanical
     equivalent of a general communication system with (classically)
     orthogonal waveforms.

The performances of QPPM systems are known only in very particular cases.
The minimum error probability for QPPM with quantum detection
 in the absence of thermal noise detection (see below) was found in
  1975 by Yuen  {\it et al.}. In 1976 Helstrom \bibll(Helstrom2)(Chapter 6)
   evaluated
   the error probability in the presence of thermal noise,
   by assuming that a classical OOK receiver counts the
   photons slot--by--slot and decides according to a majority rule.
   In 1983 Dolinar \bibl(Dolinar) suggested an adaptive measurement approach,
   called {\it conditionally nulling}, which achieves very nearly the same
   error probability of the optimum quantum  receiver in the absence of
    thermal noise. However, no precise evaluation exists in the literature
     for optimal performances of PPM in the presence of thermal noise.

\bigskip
In  QPPM the quantum--mechanical channel is
modeled by a composite Hilbert space $\C(H)$, given by the tensor
product $\C(H)_0^{\otimes m}$ of $m$ identical Hilbert spaces
$\C(H)_0$ of dimension $n$. In this space the transmitter chooses
one of $m$ pure quantum states, given by the tensor products
$$
\k(\gamma_i)=\k(\gamma_{i,m-1})\otimes\ldots\otimes\k(\gamma_{i1})
\otimes\k(\gamma_{i0})\qq i=0,\ldots,m-1\e(MF1a)
$$
where
$
\k(\gamma_{ij})=\k(\gamma^0)$ for $ j\ne i$ and
$\k(\gamma_{ij})=\k(\gamma^1)$ for $j=i$.
In a practical QPPM scheme  the two states  are assumed to be $\k(\gamma^0)=\k(0)$ (the
Glauber ground state) and $\k(\gamma^1)=\k(\alpha)$ (a Glauber state with an average number of photons $N_s=|\alpha|^2$).
The explicit constellation for  $m=4$ was given in \e(W5).
 If the states are mixed, the  composite pure states must be replaced by the
composite density operators
$$
\rho_{i}=\rho_{i,m-1}\otimes\ldots\otimes\rho_{i1}\otimes\rho_{i0}\qq i=0,
\ldots,m-1\e(MF5a)
$$
where
$
\rho_{ij}=\rho^{0}$ for $j\ne i$ and
$\rho_{ij}=\rho^{1}$ for $j=i$, and
 $\rho^{0}$ and $\rho^{1}$  are   assigned density operators on
  the space $\C(H)_0$.

\vskip-2mm


\subsection{Symmetry Operator}


The GUS structure of the QPPM constellation is apparent. Naively,
the state $\rho_{i+1}$ is obtained from $\rho_i$ through a {\co
symmetry operator} $S$ that {\co pushes
each Kronecker factor by one position (modulo $m$) to the left}.  However,
to translate the above words into a formula
 is not a
trivial problem, since the operator $S$ is not separable into a tensor
product of operators.


\Proposition(A99)  The density operators $\rho_i$ of  QPPM form
 a GUS constellation, namely $\rho_i=S^i\rho_0S^{-i}$. The symmetry
operator is given by
$$
S=\sum_{k=0}^{n-1}w_n(k)\otimes I_H\otimes
w^*_n(k)%=\sum_{k=0}^{H-1}w^*_H(k)\otimes I_n\otimes w_{H}(k)
\;,\e(P2)
$$
where $w_n(k)$ is the column vector of length
$n$, whose elements are 0 with exception of a 1 in the $k$--th
position, and $I_H$ is the identity matrix of order $H=n^{m-1}$.
\endprop

\smallskip

As an illustrative example, the symmetry operator for $n=2$
and $m=4$ (4--PPM)  takes the form
\begin{footnotesize}
$$\hbs{$S$ =}\qmatrix{
    1&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&1&0&0&0&0&0&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&1&0&0&0&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&1&0&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&1&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&0&0&1&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&0&0&0&0&1&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\cr\VS{-2}
    0&1&0&0&0&0&0&0&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&1&0&0&0&0&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&1&0&0&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&1&0&0&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&0&1&0&0&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&0&0&0&1&0&0&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0\cr\VS{-2}
    0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1\cr
}
$$
\end{footnotesize}

\noindent{\sc Proof.} The result is a particular case of a property
of the Kronecker product (see \bibl(Henderson)).
Given two matrices $A$ and $B$, with dimensions $r\times h$ and $s\times k$,
respectively, the Kronecker products $A\otimes B$ and $B\otimes A$ are different,
although they have the same dimension $rs\times hk$ and contain the same
entries,  in
different positions. Moreover, the products are related by
$$
B\otimes A=S_{rs}[\,A\otimes B\,]S_{hk}^{-1}\;,\e(P1)
$$
where the matrices $S_{rs}$ and $S_{hk}$ are permutation matrices
of order $rs$ and $hk$, respectively, known as
{\co perfect shuffle} matrices, which are independent of the
particular matrices $A$ and $B$ and depend only on their dimensions.
The matrix $S_{rs}$ is given by
$
S_{rs}=\sum_{k=0}^{s-1}\,w_s(k)\otimes I_r\otimes
w^*_s(k)
$.
Now, the symmetry operator of  QPPM gives the mapping
$$
\rho_{i,m-1}\otimes[\rho_{i,m-2}\otimes\ldots\otimes\rho_{i0}\,]\longrightarrow
[\,\rho_{i,m-2}\otimes\ldots\otimes\rho_{i0}\,]\otimes\rho_{i,m-1}
$$
which is a particular case of the general transformation \e(P1) with square matrices
$A=\rho_{i,m-1}$ of order $n$ and $B=\rho_{i,m-2}\otimes\ldots\otimes\rho_{i0}$
of order $H=n^{m-1}$. By putting  $r=h=n$ an $s=k=H$ into \e(P1), we have $S_{rs}
=S_{hk}=S_{nH}$ and we find the expression \e(P2).

\vskip-2mm


\subsection{Eigendecomposition of the Symmetry Operator}


As shown above, in the performance evaluation of a quantum detection
system that satisfies a GUS constraint,  the EID
of the symmetry operator $S$ is a key step. Since $S$ is unitary and
$S^m=I$, the EID has the form
$$
S=\sum_{k=0}^{m-1}\lambda_k\;Y_k\,Y_k^*
\e(S13)
$$
where the $Y_k$ collect, as their columns, the kets $|y_j\rangle$ corresponding
 to the eigenvalue $\lambda_k=W_m^{-k}$. The problem is the evaluation
of the matrices $Y_k$.
We can also exploit  the fact that in our case $S$
reduces to a permutation matrix. The EID of permutation matrices
is an intricate topic (see for instance \bibl(Rakosi)), at least
for the general case. However, the particular structure \e(P2) of the operator
simplifies the results.
In any case,  the {\it cycles} generated by $S$, according to the  following definition,
play a fundamental role for the EID.
Provided that $w(k)$, $k=0,\ldots,n^m-1$ are  the unit vectors of the
space $\C(H)=\C(H)^{\otimes n}$, the distinct unit vectors $w(k_0),w(k_1),
\ldots,w(k_{p-1})$ form a {\co cycle} (of {\co period} $p$) if
$S^pw(k_0)=w(k_0)$ and, for each $i=0,\ldots,p-1$, $w(k_i)=S^iw(k_0)$ .

In Appendix A we discuss the properties of the symmetry
operator $S$ listed in the following proposition.

\Proposition(P98) 1) The periods of the cycles of $S$ are
divisors of $m$. 2)
 The indexes $k_0,\ldots,k_{m-1}$ that identify
the cycle $w(k_0),w(k_1),$ $\ldots,w(k_{p-1})$ are obtained from $k_0$ through
the recursive relation
$$
k_{i+1}=nk_i \mod (n^m-1)\,.  \e(H13)
$$
3) For any cycle $w(k_0),w(k_1),\ldots,w(k_{p-1})$
the vector
$$
V_j={1\over\sqrt p}\sum_{h=0}^{p-1}W_p^{jh}w(k_h) \qq j=0,\ldots,p-1 \e(E104)
$$
is an eigenvector of $S$ associated to the eigenvalue $W_p^{-j}$.
The eigenvectors so obtained constitute an orthonormal basis of the
space $\C(H)$. \endprop


\smallskip
As a conclusion, we have the following EID of the symmetry matrix $S$
$$
S=\sum_{p\,|\,m}\sum_{c\in\C(K)_p}\sum_{j=0}^{p-1}e^{-i2\pi j/p}V_{cj}V_{cj}^*\e(E120)
$$
where the subscript $p\,|\,m$ denotes that the sum is extended to the divisors of $m$ ($m$
included), $\C(K)_p$ is the set of  cycles of minimum period $p$ and, for each cycle
$c\in\C(K)_p$, the vectors $V_{cj}$, $j=0,\ldots,p-1$ are the eigenvectors generated by
the cycle $c$. After  suitably reordering   indexes, \e(E120) can be written in the form
$$
S=\sum_{i=0}^{m-1}W_m^{-i}Y_iY_i^*\e(121)
$$
where $Y_iY_i^*$ turns out to be the projector mapping the space $\C(H)$ into the autospace associated to the eigenvalue $W_m^i$.

In order to evaluate  the EID \e(E120), we can use the following proposition,
proved in Appendix~B.

\Proposition(P95) The number $N_p$ of unit vectors of minimum period
$p$ is given by the recursive relation
$
n^p=\sum_{d\,|\,p}N_d
$.
The number of  cycles of period $p$ is $N_p/p$.
 The multiplicity of the eigenvalue
$W_m^{-h}$ is given by
$
n_h=\sum_{(m/p)\,|\,h}N_p/ p
$, $h=1,2,\ldots,m$,
where the summation is extended to all the $p$ such that $m/p$ divides $h$,
and $n_m$ gives $n_0$. \endprop


\subsection{Examples}

We reconsider the previous example of  $S$,  for $n=2$
and $m=4$ (4--PPM). The possible periods for the cycles are 1, 2, and 4.
By applying the recursive relation \e(H13), which becomes
$k_{i+1}=2k_i \mod 15$, we find the cycles $\{0\}$ and $\{15\}$ of period 1, $\{5,10\}$
of period 2, $\{1,2,4,8\}$, $\{3,6,12,9\}$, and $\{7,14,13,11\}$ of period 4.

\smallskip
The eigenvalues $1,W_4,W_4^2,W_4^3$ have 6, 3, 4, and 3 eigenvectors, respectively.
The matrices collecting the eigenvectors associated to the eigenvalues
$1,W_4,W_4^2,W_4^3$ are  then

\begin{tiny}

$$\eqalign{&\hbs{$Y_0=$}
\left[
\begin{array}{cccccc}
 1 & 0 & 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & \frac{1}{2} & 0 & 0 \\
 0 & 0 & 0 & \frac{1}{2} & 0 & 0 \\
 0 & 0 & 0 & 0 & \frac{1}{2} & 0 \\
 0 & 0 & 0 & \frac{1}{2} & 0 & 0 \\
 0 & 0 & \frac{1}{\sqrt{2}} & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & \frac{1}{2} & 0 \\
 0 & 0 & 0 & 0 & 0 & \frac{1}{2} \\
 0 & 0 & 0 & \frac{1}{2} & 0 & 0 \\
 0 & 0 & 0 & 0 & \frac{1}{2} & 0 \\
 0 & 0 & \frac{1}{\sqrt{2}} & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 & 0 & \frac{1}{2} \\
 0 & 0 & 0 & 0 & \frac{1}{2} & 0 \\
 0 & 0 & 0 & 0 & 0 & \frac{1}{2} \\
 0 & 0 & 0 & 0 & 0 & \frac{1}{2} \\
 0 & 1 & 0 & 0 & 0 & 0
\end{array}
\right]\vq
\hbs{$Y_1=$}\left[
\begin{array}{ccc}
 0 & 0 & 0 \\
 -\frac{i}{2} & 0 & 0 \\
 -\frac{1}{2} & 0 & 0 \\
 0 & -\frac{i}{2} & 0 \\
 \frac{i}{2} & 0 & 0 \\
 0 & 0 & 0 \\
 0 & -\frac{1}{2} & 0 \\
 0 & 0 & -\frac{i}{2} \\
 \frac{1}{2} & 0 & 0 \\
 0 & \frac{1}{2} & 0 \\
 0 & 0 & 0 \\
 0 & 0 & \frac{1}{2} \\
 0 & \frac{i}{2} & 0 \\
 0 & 0 & \frac{i}{2} \\
 0 & 0 & -\frac{1}{2} \\
 0 & 0 & 0
\end{array}
\right]\cr
&\hbs{$Y_2=$}\left[
\begin{array}{cccc}
 0 & 0 & 0 & 0 \\
 0 & -\frac{1}{2} & 0 & 0 \\
 0 & \frac{1}{2} & 0 & 0 \\
 0 & 0 & -\frac{1}{2} & 0 \\
 0 & -\frac{1}{2} & 0 & 0 \\
 -\frac{1}{\sqrt{2}} & 0 & 0 & 0 \\
 0 & 0 & \frac{1}{2} & 0 \\
 0 & 0 & 0 & -\frac{1}{2} \\
 0 & \frac{1}{2} & 0 & 0 \\
 0 & 0 & \frac{1}{2} & 0 \\
 \frac{1}{\sqrt{2}} & 0 & 0 & 0 \\
 0 & 0 & 0 & \frac{1}{2} \\
 0 & 0 & -\frac{1}{2} & 0 \\
 0 & 0 & 0 & -\frac{1}{2} \\
 0 & 0 & 0 & \frac{1}{2} \\
 0 & 0 & 0 & 0
\end{array}
\right]
\vq\;\;
\hbs{$Y_3=$}\left[
\begin{array}{ccc}
 0 & 0 & 0 \\
 \frac{i}{2} & 0 & 0 \\
 -\frac{1}{2} & 0 & 0 \\
 0 & \frac{i}{2} & 0 \\
 -\frac{i}{2} & 0 & 0 \\
 0 & 0 & 0 \\
 0 & -\frac{1}{2} & 0 \\
 0 & 0 & \frac{i}{2} \\
 \frac{1}{2} & 0 & 0 \\
 0 & \frac{1}{2} & 0 \\
 0 & 0 & 0 \\
 0 & 0 & \frac{1}{2} \\
 0 & -\frac{i}{2} & 0 \\
 0 & 0 & -\frac{i}{2} \\
 0 & 0 & -\frac{1}{2} \\
 0 & 0 & 0
\end{array}
\right]\cr}
$$
\end{tiny}


As another example, let $n=2$ and $m=10$, so that $n^m=1024$. The possible periods
 for the cycles are $p=1,2,5,10$. The number of  unit vectors with period $p$ are $N_1=2$,
$N_2=2$, $N_5=30$, and $N_{10}=990$. The numbers $N_p/p$ are $2,1,6,99$, respectively.
 The matrices $Y_i$ have dimension $1024\times n_i$, where  $n_0=108$,
 $n_1=n_3=n_7=n_9=99$, $n_2=n_4=n_6=n_8=105$, and  $n_5=100$.


It can be shown that the sizes of the matrices involved increase very rapidly.
 Fortunately, the matrices $Y_i$ are very sparse
  and  strongly structured. Several
  appropriate tricks can then be exploited  to alleviate the computational complexity.

\vskip-2mm



\section{Quantum states in coherent optical communications}


    In quantum optical communication systems the
correct setting of quantum states is provided by
the  Glauber's celebrated theory \bibl(Glauber). In the case of PPM,
this theory will provide the basic density operators
$\rho^0$ and $\rho^1$, representing the symbols 0 and 1, from which
 the $m$  density operators $\rho_i$ can be obtained by
tensorial products.

\vskip-2mm


\subsection{Density Operators from Glauber's Theory}


In this theory, a {\it coherent state}, representing  a monochromatic
 electromagnetic radiation produced by a  laser, is formulated in an
 infinite dimensional Hilbert space $\C(H)$ equipped with an orthonormal basis
 $|n\rangle, n=0,1,2,\ldots$, where $|n\rangle$  are called
{\it number eigenstates}. Each state $|n\rangle$ is said
to contain exactly $n$ photons. In this context the Glauber representation
 of a single  radiation mode is given by the ket
$$
|\alpha \rangle = e^{-\frac{1}{2}|\alpha|^2}
\sum_{n=0}^{\infty}{\frac{\alpha^n}{\sqrt{n!}}} |n\rangle
\e(P2a)
$$
where $\alpha$ is the complex envelope that specifies  the mode
and $N_\alpha=|\alpha|^2$ represents the {\it average number of photons}, when the
system is in
  the coherent state $|\alpha \rangle$.


The representation  \e(P2a) is valid  when the
receiver observes a pure state with a known parameter $\alpha$, which in the
context of communications may be regarded as the {\it signal}. In the presence
of thermal (or background) noise, the signal  becomes uncertain and must
be represented through a density operator. In this case the Glauber theory
provides an infinite matrix representation $||\rho_{mn}||$ of the density
 operator, given (for $0\leq m\leq n$) by
$$\eqalign{
\rho_{mn}(\alpha)&=(1-v)v^n \sqrt{\frac{m!}{n!}} \left(
\frac{\alpha^*}{\C(N)} \right)^{n-m}\! \!\!\!e^{-(1- v)|\alpha|^2
}\cdot\cr
&\;\qqq \cdot L_{m}^{n-m} \left(- \frac{|\alpha|^2}{\C(N)(\C(N)+1)} \right)\cr}
\e(C20A)
$$
where $\C(N)$ represents the {\it  average number of photons}
associated with the thermal noise, $v=\C(N)/(1+\C(N))$,
 and $L_{m}^{n-m}(x)$ are  generalized Laguerre
polynomials. The entries  for $m> n$ are obtained by
$\rho_{nm}(\alpha)=\rho_{mn}^*(\alpha)$.
The diagonal elements $\rho_{mm}(\alpha)$  obey a Laguerre distribution
and give the probabilities
 of exactly $m$ photons being present,  when the
quantum system is
in the noisy state represented by the density operator $\rho(\alpha)$ \bibl(Helstrom).
For the ground state $|\gamma\rangle= |0\rangle$  the above expression
 degenerates and the corresponding matrix representation
 becomes diagonal, namely
$
    \rho_{mn}(0)=\delta_{mn}(1-v)v^n
   $.

The infinite dimensional matrix  $||\rho_{mn}(\alpha)||,0\leq m,n<
\infty$ gives a correct representation of the density operator,
but, for practical calculations,  we introduce a finite dimensional approximation by
  truncating to $n_\epsilon$ terms.
For the choice of $n_\epsilon$, to achieve a given accuracy,
we follow the  {\it quasi--unitary trace criterion}, proposed in \bibl(CarPier), which is
based on the fact that a  density operator has  unitary trace.
Then,  we choose $n_\epsilon$ as the smallest integer,  such that
$
\sum_{m=0}^{n_\epsilon-1}
              \rho_{mm}(\alpha)\geq 1-\epsilon
$,
where  $\epsilon$ is the required accuracy. Thus, for a given $\epsilon$,
$n_\epsilon$ can be evaluated using the Laguerre
distribution $\rho_{mm}(\alpha)$.

\ev{Numerical accuracy}  The above numerical approach
implies a twofold approximation. First, the truncation of the
infinite matrix to a finite  $n_\epsilon\times n_\epsilon$  matrix $\rho$.
It is reasonable to
think that, at the increasing of $n_\epsilon$ , the approximate
 results converges to the correct ones. However,
 the evaluation of the  corresponding error seems to be a difficult
problem and we made no attempt to evaluate it. A second approximation
is that the truncated density matrix is not normalized to
unitary trace. Of course,  it can be normalized as $\bar\rho=c\,\rho$,
where $c=1/\Tr(\rho)\leq 1/(1-\epsilon)$. In the PPM the truncation is operated on the
basic operators $\rho^0$ and $\rho^1$, which we normalize as
 $\bar{\rho}^{\,0}=c\,\rho^0$ and $\bar{\rho}^{\,1}=c\,\rho^1$. To see the
 non normalization effect on the error probability $P_e=1-P_c$, we consider the
 SRM approach stated by \proposition(DFT), and mark with a bar the
 quantities obtained from  normalized density operators. For the reference
 factor we get $\bar\gamma_0=c^{m/2}\,\gamma_0$ and for the square--root
 matrices $\bar E_k^{1/2}=c^{m/2}\,E_k^{1/2}$, and finally from \e(P25)
 $\bar P_c=c^m\,P_c$. Hence,  $\bar P_e=(1-c^m)+c^m\,P_c$ and, considering
 that $\epsilon\ll 1$ and $P_e\ll 1$, we find $P_e-\bar P_e\simeq
 m \epsilon$. In conclusion, if we choose $\epsilon\ll P_e$, we see that
normalization is irrelevant.  In the numerical evaluation of Section V,
 where $P_e>10^{-6}$,
we have chosen $\epsilon=10^{-8}$.
\vskip-2mm


\subsection{Factorization of the density operators. Choice of the rank}

Once  the finite $n_\epsilon\times n_\epsilon$ approximation
 of the density operator has been established,  we need
  a factorization of the form
$
  \rho(\alpha) =\gamma(\alpha)\gamma^*(\alpha)
  $
  for a suitable  matrix $\gamma(\alpha)$.
       For $\alpha=0$ (ground state) the factorization
                is immediate, since $\rho(0)$ is diagonal, and
                 we find $ \gamma(0)
                  =\sqrt{\rho(0)}=||\delta_{mn}\sqrt{(1-v)v^n} || $.
 For $\alpha\neq0$ we evaluate
 the reduced EID of $\rho(\alpha)$, namely
$
\rho(\alpha)
=Z_h\Lambda_h^2 Z_h^*
$,
where $h$ is the rank of $\rho(\alpha)$, $Z_h$  is  an $n_\epsilon\times h$ matrix
that  collects the eigenvectors
corresponding to the $h$ positive eigenvalues $\lambda_i^2$,
 and  $\Lambda_h^2$ is the
$h\times h$ diagonal matrix that collects the $\lambda_i^2$.
Hence,
$
\gamma(\alpha)=Z_h\Lambda_h
$
is a  factor of $\rho(\alpha)$.

A critical step in the numerical evaluation is the choice of the rank $h$,
 given by the number
of numerically relevant  eigenvalues. To clarify the problem
we develop a specific case:
$
 \alpha=\sqrt5\vl N_s=5\vl \C(N)=0.1\vl\epsilon=10^{-5}\q\arr\q
 n_\epsilon=20
$. Now, in theory, $\rho(\alpha)$ has
  full rank $h=n_\epsilon$, as  can be  seen from the list of its eigenvalues,
 obtained with a high accuracy
\begin{footnotesize}
$$
\eqalign{
&0.150285\vl\;\; 0.00231095\vl\;\; 0.0000353779\vl\;\;
          5.20725\; 10^{-7}  \cr
&7.24874 \; 10^{-9}
   \vl\;\;9.45157 \;10^{-11}\vl\;\; 1.14603\; 10^{-12} \;\;\vl\ldots\cr
&3.10867 \;10^{-21}   \vl\;\;
 2.32186\; 10^{-21}   \vl\; 1.37631\; 10^{-22}   \vl\; 3.01775\; 10^{-25}\cr
 }
$$
\end{footnotesize}%
but  in practice, we can limit the list  to the first 3 eigenvalues,
neglecting the rest, which means that
 we assume $h=3$ as a ``practical'' rank. As a check, the reconstruction
 of $\rho(\alpha)$ obtained in this  way assures an accuracy $<10^{-8}$.
 To find the ``practical'' rank in the general case, we consider the reconstruction
error
$\Delta\rho=\rho-\gamma_h\gamma^*_h$,
where  the factor $\gamma_h$ is obtained by taking only $h$ eigenvalues.
Then, we can  evaluate the maximum error, or the mean square error,
 as a function of $h$ and choose $h=h_\nu$ to achieve a given accuracy
$\nu$ (for a detailed discussion of $n_\epsilon$ and $h_\nu$ versus the accuracies
$\epsilon$ and $\nu$, see
\bibl(CarPier)).

\vskip-2mm

\section{Application examples}

We apply the theory of the previous sections to  evaluate
 the error probability in QPPM systems. But first we compare
the developed methods to give a guide to
possible ranges in the different numerical evaluations.


\vskip-2mm


\subsection{Comparison of computational methods}

In the previous section, we saw that, given the accuracies $\epsilon$ and $\nu$,
we can evaluate the basic density operators
$\rho^0 =\rho(0)=\gamma_h(0)\gamma_h(0)^*$ and
$ \rho^1=\rho(\alpha)=\gamma_h(\alpha)\gamma_h(\alpha)^*$ for any
choice of signal parameter $N_s=|\alpha|^2$ and of thermal
noise parameter $\C(N)$ (it is expedient to choose the same ``practical''
rank $h$ both for $\rho^0$ and $\rho^1$). Hence, the dimensions
and the ranks are as follows:
\bu $\gamma^0$ and $\gamma^1\!$ \q $n\times h\! $\q rank $h$,
    \q $\rho^0$ and $\rho^1$ \q $n\times n \!$\q rank $h$,
\bu $\gamma_i$ \q $N\times H$ \q rank $H$,
\q $\rho_i\q $\q $N\times N$ \q rank $H$, with $N=n^m$ and $H=h^m$,
\bu state matrix $\Gamma$\q $N\times mH$\q rank $r=mH$ (if $mH\leq N$),
\bu Gram operator $T$\q $N\times N$\q rank $mH$,
\q Gram matrix $G$\q $mH\times mH$\q rank $mH$.
\ET Having  this schedule in mind, we now compare the different evaluation methods,
considering that the practical limit is determined by the dimensions of the input data
in convex linear programming (CLP), and that in general, it is given
by the dimensions of the matrices to be eigen--decomposed.

\subsubsection{Optimal solution}

This solution is available for:
\bu  pure states ($\C(N)=0$), for any order $m$,
\bu  mixed states, for $m=2$ from Helstrom's theory, but an  $N\times N$ EID
    is required,
\bu   CLP with input the $N\times N$ density operators $\rho_i$.


\subsubsection{SRM solution}

This solution is always available, for any order $m$, for both
pure and mixed states. We have two possible approaches
\bu  via Gram operator, requires the EID of an $N\times N$ matrix,
\bu via Gram matrix, requires the EIDs of  $H\times H$ matrices.
\ET  Since $H \ll N$, we have used the Gram matrix approach,
with a practical limit for the EID computation of $H\simeq1500$. With the
CLP (Matlab toolbox LMI), we found the practical limit of the size $N$
of the input density operators to be no greater than 150. These limits refer
to a standard personal computer.

To complete the preliminaries we consider two more topics.

\ev{Error probability  with pure states}  We saw that SRM gives
the optimal solution with pure states, by virtue of the PPM's GUS. For the explicit evaluation,
we use \e(Z18), where $G_{0s}=\gamma_0^*\gamma_s=\langle\gamma_0|\gamma_s\rangle=
\langle\gamma_{00}|\gamma_{s0}\rangle\cdots\langle\gamma_{0,m-1}|\gamma_{s,m-1}\rangle$.
Recalling that  the inner product of two Glauber states   is given by \bibl(Glauber) as
$
\langle\alpha|\beta\rangle =
\exp(-\frac{1}{2}(|\alpha|^2 + |\beta|^2 -2 \alpha^* \beta))
$,
 we get $G_{0s}=1$ for $s=0$ and $G_{0s}=\exp(-|\alpha|^2)=\exp(-N_s)$
  for $s\neq0$. Hence,
from \e(P25), we have
$$
P_c=\frac1{m^2}\left(\sqrt{1+(m-1)\;e^{-N_s}}+(m-1)\sqrt{1-e^{-N_s}}\;\right)^2
\e(Q2)
$$
which is in perfect agreement with the result of \bibl(Yuen), obtained with a different approach.

\ev{Comparison with classical optical PPM} In a classical optical PPM system
based on a photon counter, the error probability was evaluated by Helstrom
\bibll(Helstrom2)(Chapter VI), using the Laguerre
distribution of photon arrivals. He found
$$
P_e=\frac1m\sum_{i=2}^m(-1)^i{m \choose i}\exp\left[
    -\frac{(1-v)(1-v^{i-1})\,N_s}{1-v^i}\right]
    $$
    where $v=\C(N)/(1+\C(N))$.






\subsection{Application to 2--PPM}

For $m=2$, we do not encounter numerical problems  because, for the range of interest,
the dimension are relatively small.
We first present the results in the absence of thermal noise (pure states),
compared with the performance of a classic optical PPM system (\Fig(KN50)), which confirms the
substantial improvement of the quantum system with respect to the classical one.


In the presence of thermal noise, for 2--PPM (as for any other binary format)
an exact evaluation is possible using Helstrom's theory (see \proposition(Hel)). This possibility
was also used to check the results obtained with the Matlab LMI toolbox.
For SRM we used the Gram matrix approach.
The results are shown in \Fig(KN36) for some values of the thermal noise parameter $\C(N)$
and show that SRM overestimates the error
probability by about 30\%,  with respect to  the optimum.
We conclude that SRM is also ``pretty good''
in the presence of thermal noise.





\subsection{Application to 3--PPM}

For $m=3$, we  encounter some numerical problems  that can
 be overcome using  the alternative approaches.
We first present our results in the absence of thermal noise (pure states),
compared with the performance of a classic optical PPM system (\Fig(KN52)). We realize the
considerable improvement of the quantum system with respect to the classical one.

In the presence of noise, we used the SRM Gram matrix approach.
The results are shown in \Fig(KN19)  as a function of $N_s$,
for some values of the thermal noise parameter $\C(N)$. To extend the error
probability range down to $10^{-5}$ we chose $n=40$, $h=8$, hence $H=8^3=512$,
which is within the limit of our computational capability. The figure also compares
quantum detection
with classical photon counter detection, and shows more than 3 decades improvement
in error probability.

Since SRM is not optimal in the presence of noise, for the 3--PPM
we tried to evaluate the minimum error probability by CLP.
As shown in
\Fig(KN17), this was feasible for a very small range of $N_s$, where the dimension
$N=n^3$ can be kept below a value of  150. Anyway, this
has permitted to show
 that the SRM gives a very small overestimate of the error
probability.






\subsection{Application to 4--PPM}

For $m=4$,  the numerical problems  become very severe
and  the comparison with the optimal case (via CLP) is not possible.
We  present the results in the absence of thermal noise (pure states),
compared with the performance of a classic optical PPM system in \Fig(KN54)  and we realize the
considerable improvement of quantum 4--PPM with respect to the classical one.

In the presence of noise,  we used the SRM Gram matrix approach.
The results are shown in \Fig(KN25)  as a function of $N_s$
for some values of the thermal noise parameter $\C(N)$. To cover the error
probability range down to $10^{-5}$ we chose $n=30$, $h=6$, hence $H=6^4=1296$,
which is at the limit of our computation capability. The figure also compares quantum detection
with classical photon counter detection and shows more than 3 decades improvement
in error probability.


\section{On the Implementation}

The problem of designing and implementing an optimal quantum receiver is a
 very difficult one also in the simplest cases, as witnessed by the history
 of the optimal detector for the quantum OOK modulation format. As known,
 the error
probability that can be obtained with a classical detector (direct photon
counter) in the absence of thermal noise is given
$
P_e=(1/2)e^{-2N_s}
$,
while the error probability achievable by optimal quantum detection (the
Helstrom bound) is
$
P_{\hbt{opt}}=(1/2)\left[1-\sqrt{1-e^{-2N_s}}\right]
$
with asymptotical approximation
$
P_{\hbt{opt}}\approx(1/4)e^{-2N_s}
$.

In 1973 Dolinar \bibl(Dolinar) proposed an optimum receiver ideally
achieving the Helstrom bound.
 Under the Dolinar's receiver it was the idea of using an adaptive detection,
 by adding to the received coherent field a time--varying feedback controlled
 field. Owing to the lack of an adequate technology
  in fast electro--optics, the realization of the Dolinar receiver was not
   possible, until in 2007 Cook {\it et al.} \bibl(Nature) demonstrated its
    feasibility in a significant range
 of physical parameters.

For a quantum PPM a natural solution could be to use an OOK receiver for a
slot--by--slot hard detection slot by slot. For pure quantum
 states $\k(0)$ and $\k(\alpha)$, a classical photon counter receiver may fail
  only in detecting the state $\k(\alpha)$. It is easy to show that the
   error probability turns out to be
$
P_e=(m/(m-1))e^{-N_s}
$.
This is an exponentially degraded performance with respect to the quantum
limit \e(Q2) having  asymptotical approximation
$
P_{\hbt{opt}}\approx(1/4)(m-1)e^{-2N_s}
$.

On the other hand, an algorithm devised by Dolinar and
 called ``conditionally nulling'' \bibl(Dolinar2)
    allows to obtain an asymptotical error probability
$
P_{\hbt{opt}}\approx(1/2)(m-1)e^{-2N_s}
$,
only double of the quantum limit. This near--optimum algorithm decides at each slot (on the basis of the previous results) whether or not to add to the incoming optical signal a negative replica of the signal corresponding to
the quantum state $\k(\alpha)$.

Unfortunately, the above considerations hold true only in the absence of thermal noise. The degradation due to thermal noise
is object of research in progress.


\vskip-2mm


\section{Conclusion}

We have examined the quantum PPM format, both in the absence (pure states) and in
the presence (mixed states) of thermal noise, using the Glauber representation
of coherent states.
  Our target was a numerical evaluation of the performance of 4--PPM,
  where the dimension of the Hilbert space reaches
ten  thousand and more. To this end, we explored all the currently
available methods, namely: exact solution, convex linear programming (CLP),
 and square root measurement (SRM), and also exploited the geometrically uniform symmetry (GUS),
 a property not considered before for the PPM,
with the goal to find the least expensive implementable solution.
 We succeeded in this, but just at
the limit, so that the methods used do not appear to be useful for higher orders, e.g., 8--PPM.
The use of CLP was limited to a small error probability range in 3--PPM.

Whenever possible, we compared
SRM with optimal detection and concluded
  that SRM is very close to optimality.
 Comparisons  with the performance of
classical  detection confirms the superiority
of the quantum detection also when the thermal noise is present.


\subsection*{Appendix A: Proof of \proposition(P98)}



Given a unit vector $w(k)$ of the composite Hilbert space
$\C(H)=\C(H)_0^{\otimes n}$, a positive integer $q$ is
a {\co period} of $w(k)$ (with reference to the operator $S$) if
$S^qw(k)=w(k)$. The minimum $p$ of periods of $w(k)$ is
its {\co minimum period}. Simple considerations guarantee
some obvious facts, such as the existence of a minimum period for
each unit vector $w(k)$ and the fact that $S^qw(k)=w(k)$, if and
only if, $p$ is a divisor of $q$. In particular, since
$S^mw(k)=w(k)$, the minimum period $p$ of each unit vector must
be a divisor of $m$.


If we use the $n$--ary representation of the integer $k$, namely,
$k=k_{m-1}n^{m-1}+\ldots+k_1n+k_0$, with $0\le k_i<m$, the permutation
$$\eqalign{
&S[\,w_n(k_{m-1})\otimes\ldots\otimes w_n(k_1)\otimes  w_n(k_0)\,]\cr
&\qq=w_n(k_{m-2})\otimes\ldots\otimes w_n(k_0)\otimes w_n(k_{m-1})\cr}
\e(PP4)
$$
can be written in the form $Sw(k)=w(h)$, where
$h=k_{m-2}n^{m-1}+\ldots+k_0n+k_{m-1}$. Since
$$
nk=\sum_{i=0}^{m-2}k_in^{i+1}+k_{m-1}+k_{m-1}(n^m-1)= h\mod(n^m-1)\;,
$$
the recursion \e(H13) holds.

Since the vectors \e(E104) satisfy the condition
$$\eqalign{SV_j
    &={1\over\sqrt p}\sum_{h=0}^{p-1}e^{i2\pi jh/p}Sw(k_h)\cr
        &={1\over\sqrt p}\left[
\sum_{h=0}^{p-2}e^{i2\pi jh/p}w(k_{h+1})+e^{i2\pi j(p-1)/p}w(k_0)\right]\cr
    %\cr&=e^{i2\pi j/p}{1\over\sqrt p}\left[\sum_{h=1}^{p-1}e^{-i2\pi jh/p}w(k_h)+w(k_0)\right]
        &=e^{-i2\pi j/p}V_j\cr
    }
$$
$V_j$ is an eigenvector of $S$ associated to the eigenvalue $W_p^{-j}=e^{-i2\pi j/p}$.
Since $w^*_{k_i}w_{k_j}=\delta_{ij}$, it can be immediately verified that the
eigenvectors corresponding to a single cycle are orthonormal. Moreover, eigenvectors
corresponding to different cycles are orthogonal, in that they are
linear combinations of disjoint sets of unit vectors. Then,
item 3) follows.


\subsection*{Appendix B: Proof of \proposition(P95)}


By examining the permutation \e(PP4), it turns out that the unit vector $w(k)$
has period $d$ (not necessarily minimum), if and only
if, the $n$--ary $k_0k_1\ldots k_{m-1}$ representation of the index $k$
is periodic, of period $d$, with respect to the cyclic shift, i.e., it
is given by the concatenation of $m/d$ equal subsequences
$k_0k_1\ldots k_{d-1}$.
Since the number of such subsequences is $n^d$, this is also the
number of unit vectors with period $d$. Since a unit vector
has period $d$, if and only if, its minimum period divides $d$,
the recursion $
n^p=\sum_{d\,|\,p}N_d
$
follows. Moreover, for each subsequence $k_0k_1\ldots k_{d-1}$, its $d$
cyclic shift give rise to the same cycle, so that the number of cycles of
period $d$ is $N_d/d$.
Finally, the multiplicity is stated from the fact that a cycle of period $p$ gives rise to an
eigenvector associated to $W_m^{-h}$, if  and only if, there exists an integer $r$ such that
$W_m^{-rm/p}=W_m^{-h}$, i.e., if and only if, $h$ is a multiple of $m/p$.


\subsection*{Acknowledgment} The authors wish to thank A. Assalini, R. Corvaja,
 and P. Kraniauskas for stimulating discussions and helpful comments.

\bozzefalse

